VERN: Vegetation-aware Robot Navigation in Dense Unstructured Outdoor Environments

We propose a novel method for autonomous legged robot navigation in densely vegetated environments with a variety of pliable/traversable and non-pliable/untraversable vegetation. We present a novel few-shot learning classifier that can be trained on a few hundred RGB images to differentiate flora that can be navigated through, from the ones that must be circumvented. Using the vegetation classification and 2D lidar scans, our method constructs a vegetation-aware traversability cost map that accurately represents the pliable and non-pliable obstacles with lower, and higher traversability costs, respectively. Our cost map construction accounts for misclassifications of the vegetation and further lowers the risk of collisions, freezing and entrapment in vegetation during navigation. Furthermore, we propose holonomic recovery behaviors for the robot for scenarios where it freezes, or gets physically entrapped in dense, pliable vegetation. We demonstrate our method on a Boston Dynamics Spot robot in real-world unstructured environments with sparse and dense tall grass, bushes, trees, etc. We observe an increase of 25-90% in success rates, 10-90% decrease in freezing rate, and up to 65% decrease in the false positive rate compared to existing methods.

==> 8_Acknowledgement.tex <==
\section{Acknowledgement}

This work was supported by the U.S. Army Combat Capabilities Development Command (DEVCOM) Army Research Laboratory (ARL) Artificial Intelligence and Autonomy for Multi-Agent Systems (ArtIAMAS) program through a cooperative agreement (https://artiamas.umd.edu) and is being partially funded by DEVCOM ARL Grant No. W911NF2120076.  The US Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein.  The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the DEVCOM ARL or US Government.
